Learning Haptic-based Object Pose Estimation for In-hand Manipulation Control with Underactuated Robotic Hands

Unlike traditional robotic hands, underactuated compliant hands are challenging to model due to inherent uncertainties. Consequently, pose estimation of a grasped object is usually performed based on visual perception. However, visual perception of the hand and object can be limited in occluded or partly-occluded environments. In this paper, we aim to explore the use of haptics, i.e., kinesthetic and tactile sensing, for pose estimation and in-hand manipulation with underactuated hands. Such haptic approach would mitigate occluded environments where line-of-sight is not always available. We put an emphasis on identifying the feature state representation of the system that does not include vision and can be obtained with simple and low-cost hardware. For tactile sensing, therefore, we propose a low-cost and flexible sensor that is mostly 3D printed along with the finger-tip and can provide implicit contact information. Taking a two-finger underactuated hand as a test-case, we analyze the contribution of kinesthetic and tactile features along with various regression models to the accuracy of the predictions. Furthermore, we propose a Model Predictive Control (MPC) approach which utilizes the pose estimation to manipulate objects to desired states solely based on haptics. We have conducted a series of experiments that validate the ability to estimate poses of various objects with different geometry, stiffness and texture, and show manipulation to goals in the workspace with relatively high accuracy.

==> cover_letter.tex <==
Dear Editor,

We would like to submit the attached manuscript entitled “Learning
Haptic-based Object Pose Estimation for In-hand Manipulation with
Underactuated Robotic Hands” for consideration for possible publication
in the IEEE Robotics & Automation Letters. The manuscript is a re-submission of a previously rejected paper number 21-1876. 

The paper explores the use of haptics, i.e., kinesthetic and tactile sensing, for pose estimation and vision-free in-hand manipulation with underactuated hands. We propose a low-cost and flexible sensor that is mostly 3D printed along with the finger-tip and can provide contact location with moderate accuracy. Taking a two-finger underactuated hand
as a test-case, we analyze the contribution of these haptic features along with various regression models to the accuracy of the predictions. We test our approach on multiple objects with different shape, stiffness and texture.

To address the comments of the reviewers in the previous submission, we have modified the following:

- Additional test objects were included for pose estimation. One object has a rougher texture by wrapping it with sand-paper and another was printed with a soft material. The total number of tested objects is now eight.

- We have added an experimental comparison with methods that use visual feedback. In particular, we added experiments of Visual Servoing (VS) using eq. (2) and MPC that uses a vision-based transition model (MPC-Vis). The accuracy of the visual-based methods, MPC-Vis and VS, are equal to the success tolerance and, therefore, not reported. However and as expected, they exhibit slightly higher success rates than MPC-Critic due to more accurate pose feedback. Nevertheless, the results validate the proposed approach and show feasible manipulations with solely haptic feedback. 

- We have addressed the concerns of the scenario of Figure 1. We show a demonstration in which a robot arm with the underactuated hand can manipulate an object within an occluded cabinet into a target hole. In our demonstration, we assume that the position of the hole relative to the robot is known. This was mentioned in the caption. Furthermore, at the end of section VI.B, we mention that further work is required in order to sense the target hole using the available haptic feedback while having information about the general pose of the hole. This is commonly done with rigid grippers but not with underactuated ones. 
%In addition, extrinsic visual feedback can be used which is easier than observing the object in the hand with an on-board camera. 
In the introduction, we note that achieving vision-free pose estimation would enable further fusion with vision for better estimation in unstructured or partly-occluded environments.

- A comment was made regarding the novelty of our proposed FlX-finger. We have cleared this issue. In the introduction, we mention that the fingers are mostly 3D printed along with a simple off-the-shelf force Sensitive Resistors (FSR). Hence, we do not fabricate FSR sensors but use them to fabricate a finger with augmented sensing capabilities. In section VI.A, we address this issue more broadly: While the use of FSR for tactile perception is not novel (Kappassov et al., 2015), we propose a flexible 3D printed mechanism that augments the sensor and provides more contact data. When an object is being pressed against the contact pad, the flexible joint and pad deform such that different contact locations across the pad provide different voltages. Pressure on the contact pad, therefore, provides voltage signals that embed information regarding the location and magnitude of contact (presented experiments validate this). Therefore and unlike custom made force sensors (e.g., Muth et al., 2014), we use a standard off-the shelf FSR sensor and a 3D printed finger structure to acquire diverse contact data.

With the submission of this manuscript I would like to undertake that the above mentioned manuscript has not been published elsewhere, accepted for publication elsewhere or under editorial review for publication elsewhere; and that my institute’s representative is fully
aware of this submission.
